Generalization through Diversity: Improving Unsupervised Environment Design

Agent decision making using Reinforcement Learning (RL) heavily relies on either a model or simulator of the environment (e.g., moving in an 8x8 maze with three rooms, playing Chess on an 8x8 board). Due to this dependence, small changes in the environment (e.g., positions of obstacles in the maze, size of the board) can severely affect the effectiveness of the policy learned by the agent. To that end, existing work has proposed training RL agents on an adaptive curriculum of environments (generated automatically) to improve performance on out-of-distribution (OOD) test scenarios. Specifically, existing research has employed the potential for the agent to learn in an environment (captured using Generalized Advantage Estimation, GAE) as the key factor to select the next environment(s) to train the agent. However, such a mechanism can select similar environments (with a high potential to learn) thereby making agent training redundant on all but one of those environments. To that end, we provide a principled approach to adaptively identify diverse environments based on a novel distance measure relevant to environment design. We empirically demonstrate the versatility and effectiveness of our method in comparison to multiple leading approaches for unsupervised environment design on three distinct benchmark problems used in literature.

==> rebuttal.tex <==
% author response 

\section*{Rebuttal}
\textbf{Reviewer \#1}\\
We thank the reviewer for the positive and constructive remarks.\\
\textbf{Q1.} Can DIPLR handle problems with varying level sizes, and learn/generalize from small levels to large levels? \\
\textbf{A1.} Since we are using the occupancy measure induced by agent trajectories, which is level-structure-agnostic and level-size-agnostic, DIPLR can effectively compute the diversity with varying level sizes. \\


\noindent
\textbf{Reviewer \#2}\\
We thank the reviewer for the positive and constructive remarks.\\
\textbf{Q1.} Would it be possible to show results for running DIPLR with regret alone? That might further provide evidence that both are needed. \\
\textbf{A1.} Please note that:
DIPLR: regret + diversity;
DIPLR$^-$: diversity;
PLR$^\perp$: regret alone.
So, please note that the current graphs already have these results. \\

\noindent
\textbf{Reviewer \#3}\\ 
We thank the reviewer for the very positive and valuable feedback. We will fix the mentioned issues in the revised version. \\

\noindent
\textbf{Reviewer \#4}\\
We thank the reviewer for the feedback and request to consider the small misunderstanding with regard to UED and RL. 

There seems to be a fundamental misunderstanding with regard to the use of diversity in Unsupervised Environment Design (UED) versus diversity in  Reinforcement Learning (RL). 
In research works on diversity in RL, the focus is on finding ``diverse policies" to improve ``exploration" on a "single level". On the other hand, in our paper on diversity in UED, the focus is on finding ``diverse levels" to train an ``agent policy" to ``generalize better" across levels.  Because of this difference, the former requires distance between behaviors or policies, while the latter requires distance between environments/levels. 

We request the reviewer to please consider the above paragraph, as most of the comments seem to be connected to the above difference in understanding. 

Q1. ``Hence, this work relies on measuring trajectories of the same student policy in different environments which is different from maximizing the generalization capability of a student agent."

A. Measuring distance between trajectories of the same student policy in different environments helps us compute diversity between environments given the current policy. Our hypothesis is that getting more diverse environments will lead to improvement in generalization ability. This is intuitive, as the more varied experiences we have, our decision making becomes more generalizable. 

Q2. Hong et al. 2018, Parker-holder et al. 2020, Lupu et al. 2021

A. Please refer to the initial paragraph of the response. All these references are on diversity in RL. 


Q3. Type of diversity approach.

A. UED is different from regular RL. To the best of our knowledge, diversity across levels (and not across policies/behaviors like in RL) has not been explored previously. More importantly, those approaches employed for diversity in RL cannot be directly extended to our problem, as each level is like a different RL problem. Also, please note that we have one current policy and we are evaluating diversity across levels from the context of that policy. 

Q4. Why not compare against diversity in RL approaches?

A. Diversity in RL approaches is for increasing exploration within one level. In UED, we are trying to expose the student agent to multiple diverse levels. So, those approaches are not applicable in our context. 

Q5. Why not use JSD instead of Wasserstein?

A. It is well known that Wasserstein is a more stable distance metric, which is also the main reason why Wasserstein is now being utilized in imitation learning and in adversarial learning. More importantly, to compute JSD, we need explicit density functions that we do not have in our setting. A nice property of Wasserstein distance is that it can measure the distance between two distributions based on only data samples.

Q6. ``regret and GAE for level generation and it is known that high regret environments do not guarantee sufficiently different levels."

A. Actually, to the best of our knowledge, this was not known earlier and was not mentioned in existing works. This insight is something we provide in this paper. 

Q7. Irreproducible?

A. We have provided the pseudocode of DIPLR and included our implementation in the technical appendix. Reproducing our results is not a problem, especially since our implementation is based on the most popular and stable codebase in the UED community. We will also be open-sourcing our implementation and give detailed hyperparameters in the updated draft. 





% \textbf{Paragraph-3: The paper is unclear about...}
% None of the related works on diversity in RL can be directly extended to our problem. The (1) approach is specifically targeted at transfer RL, where the agent policy is trained in a particular task domain and then transfer to another different task domain (e.g. from walking with four legs to walking with two legs). This kind of comparison is to explore the exact difference between two domains, and is independent of agent policy. There won't be any difference between two particular levels if we adopt this approach because the comparison is conducted in the same task domain. The (2) approach that explores either pair-wise difference or population-wise difference between policies is also not applicable to our problem. In UED, we want to obtain a single robust agent policy through open-ended level generation. We achieve this goal by promoting diversity in training levels, rather than increasing the number of agent policies or promoting their diverse behaviors. To the best of our knowledge, there is no paper exploring UED with a population of agent policies and thus we do not have multiple agent policies to compare. \\
% (The setting of environment design is different from traditional RL, as its focus is on developing a sequence of environments to train a robust agent. Consequently, the two existing methods used to assess diversity in RL are not directly transferable to evaluate the diversity of environments in our problem.) \\
% \textbf{Paragraph-4: In the same line...}
% The following references [Hong et al 2018, Parker-Holder et al 2020, Lupu et al 2021] are not in the field of UED and their objective is to promote diverse behaviors in agent policies. In contrast, our method computes the distance between levels and thus is not comparable to these referred papers. Moreover, JSD is not applicable to our problem. To compute JSD, we need explicit density functions that we don't have.  \\
% \textbf{Paragraph-5: Regarding the obtained results...}
% We agree with your hypothesis that purely adversarial RL is not suitable in UED. When you look at the trajectory of works in UED, the latter algorithms all adopt domain randomization as the generation method and then connect with various techniques to find high-potential levels, e.g. use GAE-based regret to filter out low-potential levels or employ human-specified edits to gradually improve level complexity. We didn't discuss this in detail because it's not our main contribution
% and we are also restricted by the IJCAI page limit.\\

% \textbf{Reproducible Results}



